Completeness Theorems for k-SUM and Geometric Friends: Deciding Fragments of Integer Linear Arithmetic

In the last three decades, the $k$-SUM hypothesis has emerged as a satisfying explanation of long-standing time barriers for a variety of algorithmic problems. Yet to this day, the literature knows of only few proven consequences of a refutation of this hypothesis. Taking a descriptive complexity viewpoint, we ask: What is the largest logically defined class of problems \emph{captured} by the $k$-SUM problem? To this end, we introduce a class $\mathsf{FOP}_{\mathbb{Z}}$ of problems corresponding to deciding sentences in Presburger arithmetic/linear integer arithmetic over finite subsets of integers. We establish two large fragments for which the $k$-SUM problem is complete under fine-grained reductions: 1. The $k$-SUM problem is complete for deciding the sentences with $k$ existential quantifiers. 2. The $3$-SUM problem is complete for all $3$-quantifier sentences of $\mathsf{FOP}_{\mathbb{Z}}$ expressible using at most $3$ linear inequalities. Specifically, a faster-than-$n^{\lceil k/2 \rceil \pm o(1)}$ algorithm for $k$-SUM (or faster-than-$n^{2 \pm o(1)}$ algorithm for $3$-SUM, respectively) directly translate to polynomial speedups of a general algorithm for \emph{all} sentences in the respective fragment. Observing a barrier for proving completeness of $3$-SUM for the entire class $\mathsf{FOP}_{\mathbb{Z}}$, we turn to the question which other -- seemingly more general -- problems are complete for $\mathsf{FOP}_{\mathbb{Z}}$. In this direction, we establish $\mathsf{FOP}_{\mathbb{Z}}$-completeness of the \emph{problem pair} of Pareto Sum Verification and Hausdorff Distance under $n$ Translations under the $L_\infty$/$L_1$ norm in $\mathbb{Z}^d$. In particular, our results invite to investigate Pareto Sum Verification as a high-dimensional generalization of 3-SUM.

==> Appen.tex <==
%\appendix 
\section{Baseline Algorithms} \label{sec:baseline}
\begin{lemma}
Every problem in the class $ \mathsf{FOP}_{\mathbb{Z}}(\exists^k)$ can be decided in time $\tilde{O}(n^{\lceil k/2 \rceil})$.
\label{baseline_exist}
\end{lemma}
\begin{proof}
    To this end, after substituting the free variables $\hat{t_1}, \dots \hat{t_l}$ in the quantifier free part of $\phi$, without loss 
    of generality, by the same arguments used in the proof of Theorem \ref{existential_complete}, we can transform every such linear arithmetic formula $\phi[(t_1,\dots,t_l)\backslash(\hat{t_1},\dots,\hat{t_l})]$ into the following form:
    $$\exists a_1 \in A_1 \dots \exists a_k \in A_k:\bigvee_{h=1}^{H}\bigwedge_{i=1}^{m} \sum_{j=1}^{k}c_{h,i,j}^T  a_j \geq S_{h,i}.$$
    Due to the commutativity of disjunction and existential quantifiers, we can rewrite the above in the form:
    $$ \bigvee_{h=1}^{H}\exists a_1 \in A_1  \dots \exists a_k \in A_k:\bigwedge_{i=1}^{m} \sum_{j=1}^{k}c_{h,i,j}^T  a_j \geq S_{h,i}.$$
    Now it suffices to have a look at $H$ instances of the following problem, whose results are combined disjunctively
    $$\exists a_1 \in A_1  \dots \exists a_k \in A_k:\bigwedge_{i=1}^{m} \sum_{j=1}^{k}c_{i,j}^T  a_j \geq S_i,$$
    where $S_i \in \mathbb{Z},c_{i,j} \in \mathbb{Z}^{d_j}.$
    Consider summing up the tuples by their corresponding coefficients, that is we consider the sets 
\begin{align*}
  A_j^{'}:=\left\{ \left(\begin{array}{c}
  c_{1,j}^T a  \\
  c_{2,j}^T a \\
  \vdots  \\
  c_{m,j}^T a
  \end{array}\right)   : a \in A_j \right\},
\end{align*}
and define $S:=(S_1,S_2,\dots,S_m)^T$.
We are now left with the following problem
\begin{align*}
\exists a_1' \in A_1' \dots \exists a_k' \in A_k': \sum_{j=1}^{\lceil k/2 \rceil }a_j' \geq \sum_{j=\lceil k/2 \rceil +1}^{ k } a_j' + S
\end{align*}
Precompute the left-hand side sums and the right-hand side sums in $O(n^{\lceil k/2 \rceil })$. Store all possible sums in the left-hand side in a range tree, see \cite{DBLP:conf/focs/AlstrupBR00}.  Iterating over the precomputed sums in the right-hand side and querying them in the range tree gives us an algorithm in time $\Tilde{O}(n^{\lceil k/2 \rceil })$.
\end{proof}

\begin{lemma}
Every formula $\phi$ in one of the classes $$\FOPZ(\exists \exists),\FOPZ(\forall \forall),\FOPZ(\exists \forall ),\FOPZ(\forall \exists),$$
can be decided in time $\Tilde{O}(n)$.  \label{baseline:twoquant}
\end{lemma}
\begin{proof}
If $\phi$ is in the class $\FOPZ(\exists \exists)$, we can conclude by the same algorithm as in Lemma \ref{baseline_exist}.
If $\phi$ is in the class $\FOPZ(\forall \exists)$, after substituting the free variables, by the same arguments used in the proof of Theorem \ref{existential_complete}, we can transform $\phi$ to an equivalent formula of the type:
$$\forall a_1 \in A_1 \exists a_2 \in A_2:\bigvee_{h=1}^{H}\bigwedge_{i=1}^{m} c_{h,i,1}^T  a_1+ c_{h,i,2}^T a_2 \geq S_{h,i},$$
which is equivalent to 
$$\forall a_1 \in A_1 \bigvee_{h=1}^{H} \exists a_2 \in A_2:\bigwedge_{i=1}^{m} c_{h,i,1}^T  a_1+ c_{h,i,2}^T a_2 \geq S_{h,i}.$$
Consider 
\begin{align*}
  A_2^{(h)}:=\left\{ \left(\begin{array}{c}
  c_{h,1,2}^T a  \\
  c_{h,2,2}^T a \\
  \vdots  \\
  c_{h,m,2}^T a
  \end{array}\right)   : a \in A_2 \right\},
\end{align*}
$S^{(h)}:=(S_{h,1},\dots,S_{h,m})^T$, and finally $a_1^{(h)}:=(c_{h,1,1}^T a_1,c_{h,2,1}^T a_1, c_{h,m,1}^T a_1)$.
Then, it remains to solve:
$$\forall a_1 \in A_1 \bigvee_{h=1}^{H} \exists a_2 \in A_2^{(h)}: a_2 \geq S^{(h)} -a_1^{(h)}.$$

Thus, we insert in $H$ different orthogonal range trees, the elements of $A_2^{(h)}$.

By iterating over all the elements in $A_1$, and checking whether for any $h \in \{1,\dots,H\}$, the vector $S^{(h)}-a_1^{(h)}$ is dominated by some $a_2 \in A_2^{(h)}$ via a range tree query,
we can conclude. 

Finally, by simply negating the formula and pushing the negation inwards, we can always get a formula in $\FOPZ(\exists \exists)$ or $\FOPZ(\forall \exists)$.
\end{proof}
\begin{lemma}
  Every problem in the class $\mathsf{FOP}_{\mathbb{Z}}^k$ can be decided in time $\Tilde{O}(n^{k-1})$.
\label{baseline} 
\end{lemma}
  \begin{proof}
  Let $\phi$ be in $\mathsf{FOP}_{\mathbb{Z}}$.
  After substituting the free variables, we brute force the first $k-2$ quantifiers. It remains to solve a formula 
 $\varphi$ with 2 quantifiers. We can conclude by a simple application of Lemma \ref{baseline:twoquant}
\end{proof}


%\section{Continuation of Preliminaries} \label{appencontinuation}

\section{Proof of Lemma \ref{Ineq_to_eq}}\label{lemma_conj_ineq}
\begin{proof}
    We define the transformations for $f^{\ell,\psi}_j$ with $j \in \{1,\dots,k\}$ and the transformation $g^{\ell,W,\psi}$  as the following vectors with $2m$ dimensions:
     \begin{flalign*}
     \underbrace{ \left(\begin{array}{c}
       pre_{\ell[1]}(M+p_{1,j}( a_j))  \\
       \vdots  \\
       pre_{\ell[m]}(M+p_{m,j}( a_j))\\
       pre_{\ell[1]-1}(M+p_{1,j}( a_j)) \\
       \vdots \\
       pre_{\ell[m]-1}(M+p_{m,j}( a_j))
       \end{array}\right)}_{=:f^{\ell,\psi}_j(a_j)} \quad\quad       \underbrace{ \left(\begin{array}{c}
        pre_{\ell[1]}\left(S_1-1+ kM \right)+W[1] \\
        \vdots  \\
        pre_{\ell[m]}(S_m-1+ kM)+W[m]\\
        pre_{\ell[1]-1}\left(S_1-1+ kM \right) \\
        \vdots  \\
        pre_{\ell[m]-1}(S_m-1+ kM)
        \end{array}\right).}_{=:g^{\ell,W,\psi}(S_1,\dots,S_m)}
     \end{flalign*}

     Notice that $pre_\ell$ is applied on non-negative integers due to the choice of $M.$
     For all $\ell \in \{1,\dots,\lceil \log_2(M) \rceil \}^m, W \in \{1,\dots,k\}^m$, we have that 
     \begin{align*}
       & f^{\ell,\psi}_1 (a_1)+\dots + f^{\ell,\psi}_k (a_k)=g^{\ell,\psi,W} (S_1,\dots,S_m) \\
       \iff &  \underbrace{\bigwedge_{i=1}^m \sum_{j=1}^{k} pre_{\ell[i]}(M+p_{i,j}( a_j))= pre_{\ell[i]}\left(S_i-1+ kM \right)+W[i]}_{=:\varphi_1(\ell,W)} \\
       \land & \underbrace{\bigwedge_{i=1}^m \sum_{j=1}^{k} pre_{\ell[i]-1}(M+p_{i,j}( a_j))= pre_{\ell[i]-1}\left(S_i-1+ kM \right)}_{=:\varphi_2(\ell,W)}.
     \end{align*}
     By Lemma \ref{bit_trick} (also Observation \ref{uniqueness_bit}), there exist unique $ \ell' \in \{1,\dots,\lceil \log_2(M) \rceil \}^m, W' \in \{1,\dots,k\}^m$ such that 
     \begin{align*}
       \varphi_1(\ell',W') \land \varphi_2(\ell',W')\iff \bigwedge_{i=1}^m\sum_{j=1}^{k} M+p_{i,j}(a_j) >S_i -1 + kM,
     \end{align*}
     which is equivalent to the desired conjunction of inequalities.
     The function of the dimensions $m+1,\dots,2m,$ and in particular $\varphi_2(\ell',W')$ are to ensure the uniqueness for the choices of $b$ and $\ell$ in Lemma \ref{bit_trick}.
   \end{proof}

\section{Proof of Disjoint boxes Lemma} \label{sec:disjointboxes}

%\begin{definition}
  %We call a collection of interior disjoint rectangles lonely if and only if each rectangle has at most one neighbor in each direction.
 % \end{definition}
  %\begin{lemma}
  %The union of $n$ overlapping squares can be decomposed into a lonely decomposition of $O(n)$ rectangles in time $O(n \log n)$.
  %\label{lemma:decomp}
  %\end{lemma}
  \begin{lemma}
	  We can decompose a rectilinear shape of complexity $n$ in $O(n)$ interior- and exterior-disjoint rectangles, some of which may be degenerate, in time $O(n \log n)$.
  \label{lem:2d}
  \end{lemma}
  \begin{proof}
  At the beginning, we aim to decompose the rectilinear shape into interior-disjoint rectangles.
  For this purpose, we perform a sweep-line algorithm. The sweep-line goes through the $x$-direction. 
  Firstly, we maintain a collection of components given by a segment in $y$ direction, which will intuitively denote the opening of components(or rectangles) which are not overlapping.
  Each vertex event, will now either create a new component, will enlarge an existing component, will shrink an existing component, or will make it disjoint. By shooting a ray up and down from this event point vertex
  we can create a new rectangle, together with the current existing component. The vertices intersected by this ray, will form the starting points for the new component.
  For details see the figure below. As each vertex will create at most one new rectangle, we conclude that the number of rectangles is in $O(n)$.
  \begin{figure}[H]
  \includegraphics[width=\textwidth, height=6cm]{decomposition.pdf}
  \caption{To the left we can find the rectilinear shape. To the right we find the decomposition into interior disjoint rectangles.}
  \end{figure}
  The rectangles formed by the above procedure are kept as open $2$-boxes.
  We now turn to the face segments of these rectangles. If a vertex event point splits a segment, we 
  decompose the segment at this point. Clearly at most $O(n)$ segments (1-boxes) can be created in this way.
  The $1$-boxes we will keep as open, and the vertices as closed $0$-boxes (or points).
\end{proof}



\begin{lemma}
	The union of $n$ unit cubes can be decomposed into $O(n)$ interior- and exterior-disjoint axis-aligned boxes, some of which may be degenerate, in time $O(n \log^2 n)$.
\end{lemma}
\begin{proof}
We adapt the algorithm of \cite{DBLP:journals/dcg/ChewDEK99} to also create exterior-disjoint boxes.
Slice the three-dimensional space by planes parallel to the $z$ axis for planes $z=1, z=2, z=3 \dots$ (without loss of generality, we can assume the cubes to be starting at $z=1$).
Consider the slab of cubes generated by cutting the cubes by  the plane $z=i$ and $z=i+1$, where we 
denote by $n_i$ the number of cubes cut by the plane $z=i$. The complexity of the slab is in $O(n_i+n_{i+1})$ by \cite{DBLP:journals/dcg/BoissonnatSTY98}.

We repeat the following for each slab.

Let $E$ be the portion of cubes that lie within the slab bounded by $z=i$ and $z=i+1$, and let the 
silhouette of $E$ be the projection on both $z=i$ and $z=i+1$ of all vertical lines whose intersection with
	$E$ is one unit long -- we refer to this vertical length as \emph{height}.

We firstly construct a decomposition of the silhouette of $E$ into interior- and exterior-disjoint boxes.
To achieve this we perform a decomposition as given in Lemma \ref{lem:2d} of the projection of the silhouette onto the plane $z=i$.
After achieving this decomposition, we create $3$-boxes out of the rectangles, with height 1, which we keep open.
Out of the segments, we create open $2$-boxes with height $1$, and from the vertices we create open $1$-boxes of height $1$.

Let $S$ be the projection of the silhouette of $E$ onto the plane $z=i$, and $S'$ be the projection of the silhouette of $E$ onto the plane $z=i+1$.
	Moreover, let $E'$ be the intersection of $E$ with the plane $z=i$, and let $F'$ denote the points on $E'$ whose vertical line length (i.e., height) changes.
	Computing $F'$ (with the associated heights) costs time $O((n_i+n_{i+1}) \log^2 (n_i+ n_{i+1}))$ by computing the union of the cubes in the slab by \cite{AgarwalS21}.


Consider $F'$ without $S$, where $S$ is the union of the formed rectangle decomposition of the silhouette of $E$.
We perform the Lemma \ref{lem:2d} decomposition onto this rectilinear shape, with the restriction that the rays shot up and down do not cross 
	$S$. Create the open $3$-boxes just like in the step for the silhouette, with the difference being that we use the height of each produced rectangle (which by construction is uniform over the rectangle).
We ignore the segments and vertices which lie adjacent to $S$ (they have height $1$ and are already taken care of).
For the remaining segments and vertices, we create open $2$-boxes and closed $1$-boxes respectively, where we take the height of the larger adjacent box. Finally, in contrast to the silhouette we also create open $2$-boxes for the faces, which lie on top of the created open $3$-boxes (or rather the face lying on the height of the $3$-box).

Proceed analogously for $E''$ which is the intersection of $E$ onto the plane $z=i+1$ and $F''$, the points on $E''$ whose vertical line length changes.

Finally, it remains to treat the rectilinear shapes $E'$ and $E''$ separately, as none of the boxes include the faces on the plane $z=i$ and $z=i+1$.
For this again, we perform the Lemma \ref{lem:2d} decomposition for $E'$ and $E''$ respectively, where we keep the rectangles and segments, as open $2$ and $1$-boxes respectively, and the vertices 
as closed $0$-boxes which lie on the respective plane.
\end{proof}


  %\section{Proofs for section 6}\label{Appendix6}
  
  %\paragraph*{Proof of Theorem \ref{HCsumset}}
  %\begin{proof}
   % On a high level the search space $[t]$ will denote all potential cliques. The reduction will transform a YES instance of $3$-uniform $6$-hyperclique into a NO instance of $[t]\subseteq A+B$.  
    %We consider the graph to be $6$-partite with node sets $V_0, \dots, V_5.$ In each of $V_0, \dots, V_5$,
    %we add two dummy vertices. The dummy nodes are not connected by an edge to any other node.
    %We number the vertices in each partition $V_0, \dots ,V_5$ from $0$ to $|V|+1$, where node $0$ and node $1$ are the dummy nodes. 
    %Consider $N :=|V|+2$, and each clique $C$ to be a number in basis $N$, for $x_{i} \in \{0,\dots,|V|+1\}$ that means:
    %$$ C:= \sum_{i=0}^{5} x_{i}\cdot N^i.$$
    %Consider $$A=\left\{\sum_{i \in I} v_i \cdot N^i: I \in \binom{[5]}{3}, \{v_i: i \in I\} \not \in E  \right\},$$
    %which is the set of numbers describing non-edges.
   % Furthermore, consider 
    %$$ B:= \left\{\sum_{i \in I}x_i\cdot N^{i} : I \in \binom{[5]}{3}, x_i \in \left[ |V|+1 \right]\right\} .$$
    %The size of $A$ is due to the size of the edges in $\Theta(n^3)$. The size of $B$ is also clearly in $\Theta(n^3)$.
    %Set $t:=N^6-1$. 
    %For the correctness let $C \in [t]$, which represents a potential clique $(c_0,\dots,c_5)$, with $c_i \in V_i$.
    %We claim that $C\in A+B$ if and only if $(c_0,\dots,c_5)$ does not form a clique.
    %Assume $C \in [t]$ represents $(c_0,\dots,c_5)$ that do not form a clique, then $C$ contains a missing edge represented by an $a \in A$ and there also exists $b \in B$ such that $C=a+b$ by construction.

    %Assume now there exists $a=\sum_{i=0}^{5} a_{i}\cdot N^i \in A, b=\sum_{i=0}^{5} b_{i}\cdot N^i \in B$ and $C= \sum_{i=0}^{5} c_{i}\cdot N^i \in [t] $ such that $a+b=C$ for some $a_i,b_i \in \{0,\dots,|V|+1\}$.
    %If there was an overflow when adding $a$ and $b$, that is $a_i+b_i>N-1$ for an $i \in [5]$. Then one of the following cases happens, there is a $j \in [5]$ with $c_j=0$, or we have some $k \in [5]$ with $a_k+b_k>N-1$ and $c_{k+1}=1$.
    %As these cases consist of at least one dummy node, $C$ is not a clique. 
    %Assume now there was no overflow when adding, that is for all $i \in [5]$ we have $a_i+b_i \leq N-1$, then there exist disjoint $I_1,I_2 \subseteq [5]$, with $I_1 \cup I_2=[5].$
    %Clearly, $\{v_i: i \in I_1\}$ is a non-edge and thereby $C$ is not a clique.
    %Assuming, there was an algorithm solving $[t] \subseteq A+B$ in time $O(n^{2-\epsilon})$ for an $\epsilon>0$, then we would get an algorithm in time $O((n^3)^{2-\epsilon})=O(n^{6-\epsilon'})$ for an $\epsilon'>0$, for the 
    %$3$-uniform $6$-hyperclique problem refuting the hypothesis.
    %\end{proof}

   % \begin{lemma}[$3$-SUM $\leq_2$ Verification of $2$-dimensional Pareto Sum]
    %  If Verification of $2D$ Pareto SUM can be solved in time $O(n^{2-\epsilon})$ for an $\epsilon>0$, then we can solve $3$-SUM in time $O(n^{2-\epsilon'})$
    %  for an $\epsilon'>0$.
    %  \end{lemma}
    %\begin{proof}
    %We reduce from the problem 
    %$$ A+B\subseteq C +[t],$$ which we have shown to be $3$-SUM hard. We define the sets $$A':= \left \{ \left(
    % \begin{array}{cc}
    %    a \\
    %    -a \\
    %    \end{array}  \right)
    %    :a \in A  \right \}.$$
   % 
    %    $$B':= \left \{ \left(
     %\begin{array}{cc}
      %  b \\
       % -b \\
        %\end{array}  \right) : b \in B
        % \right \}.$$
    
        %$$C':= \left \{ \left(
         %   \begin{array}{cc}
          %     c+t \\
           %    -c \\
            %   \end{array}  \right) : c \in C
             %   \right \}.$$
    %The quantifier structures match, and we conclude correctness by rewriting $c \leq a+b \leq c+t \iff a+b \leq c+t \land -a-b\leq -c $.
    %\end{proof}

    %\section{Continuation of Count chapter}
    




==> Problems.tex <==
\section{Examples of problems in $\mathsf{FOP}_{\mathbb{Z}}$} \label{sec:Examples}
In the following, we give a plethora of examples of problems in $\mathsf{FOP}_{\mathbb{Z}}$.
\begin{example}[3-Average free set]
Consider a finite set of integers $A$. Is there no arithmetic progression of length $3$? 
We can use the negation of the following sentence to obtain an answer.

	\[ \exists a_1 \in A \exists  a_2 \in A \exists a_3 \in A: a_1 <a_2<a_3 \land a_1 +a_3=2a_2.\]
\end{example}
We use the condition $a_1 <a_2 <a_3$ as to avoid $a_1=a_2=a_3$.
The 3-average free set problem is known to be subquadratic equivalent to $3$-SUM~\cite{DBLP:conf/stoc/0001GS20}, which itself is another example.
\begin{example}[3-SUM and Conv-3SUM]
Consider a finite set of integers $A$. Are there three numbers in $A$ summing up to $0$? I.e., 
	\[ \exists a_1 \in A \exists  a_2 \in A \exists a_3 \in A: a_1 +a_2+a_3 = 0.\]
	We can also express its subquadratic equivalent formulation convolutional $3$-SUM\footnote{For further discussion, see Section~\ref{sec:prelim}.} as a two-dimensional formula:
	Representing a  sequence $X[0 \dots n-1]$ as $X'=\{ (i,X[i]) \mid 0 \le i < n\}$, we ask whether given sequences $A[0\dots n-1],B[0 \dots n-1],C[0 \dots n-1]$ satisfy:
	\[ \exists (i,a[i])\in A' \; \exists  (j,b[j]) \in B' \; \exists (k,c[k]) \in C': a[i]+b[j]=c[k] \land i+j=k\]
\end{example}

More generally, we can view these problems as natural database queries with numerical data, e.g.: 
\begin{example}[Orthogonal Range and Database queries]
    Consider a database $\mathcal{D}$, where each entity consists of a tuple $(id,age,income)$. 
    The following query is part of the class $\mathsf{FOP}_{\mathbb{Z}}(\exists^3 )$.\\
    \emph{Do there exist three different people in $\mathcal{D}$, whose average age is below 30, whose income is in the range $[10000,20000]$, and
    whose incomes accumulate to more than $50000$?}
\end{example}

All the above examples use existentially quantified variables. This existential fragment will be of particular interest for us.

Other quantifier structures also give rise to natural algorithmic problems. 

\begin{example}[Universal $3$-SUM]
Given sets $A,B,C \subseteq \mathbb{Z}$. Does for all $a \in A $ exist $b \in B$ and $c \in C$ such that 
$c=a+b$. Clearly the problem is in $\FOPZ(\forall \exists \exists)$. Alternatively, one can also view the problem as a sumset expression, namely
$C \subseteq A+B$.
\end{example}
We note that Universal $3$-SUM seems to be a weaker version of All-ints $3$-SUM and that in general the class $\FOPZ(\forall \exists \exists)$ seems
to be the most likely to admit a subquadratic algorithm, as it has the weakest known lower bound barrier.

\begin{example}[Verification of $\Delta$-approximations of sumsets]\label{ex:addApx}
Bringmann and Nakos introduce a notion of additive approximation of sumsets in \cite{DBLP:conf/soda/BringmannN21}. We consider the problem of verifying whether a set additively approximates a sumset.  
	Specifically, let $A+B:=\{a +b: a \in A, b \in B\}$ denote the sumset of $A$ and $B$. We say that a set $C$ is an additive $\Delta$-approximation\footnote{We remark that we use here a simplified notion of additive approximation that is closely related to the ones used by Bringmann et al.~\cite{DBLP:conf/soda/BringmannN21}.} of $A+B$ whenever %for is used in the context of sumsets $A+B:=\{a +b: a \in A, b \in B\}.$

	\[
\forall a \in A \forall b  \in B\exists c \in C: c \leq a+b \leq c+\Delta \iff A+B \subseteq C+\{0,\dots,\Delta\}.
	\]
Note that we could also require each number in $C$ to be a sum itself by taking the conjunction with the Universal $3$-SUM formula:
	\[
		\forall c \in C \exists a \in A \exists b \in B: a+b=c \iff  C \subseteq A+B.\\
	\]
\end{example}
The above example makes use of the free variables in the definition of the problem $\mathsf{FOP}_{\mathbb{Z}}(\phi)$, in this case the additive approximation constant $\Delta$ is a free variable and can be instantiated by an input natural number.
Interestingly, the conjunction of both conditions $A+B \subseteq C+\{0,\dots,\Delta\}$ and $C \subseteq A+B$ can be reduced to $3$-SUM,
as $A+B \subseteq C+\{0,\dots,\Delta\}$ is in $\FOPZ(\forall \forall \exists)$ and has inequality dimension 2, and $C\subseteq A+B$ is in $\FOPZ(\forall \exists \exists)$.
\begin{example}[Hausdorff Distance under $n$ Translations]\label{ex:hunt}
We recall the definition of the Hausdorff Distance under $n$ Translations problem over $d$-dimensional sets $A,B,C$, and a value $\gamma \in \mathbb{N}$, where we ask whether the following holds
 \[\delta_{\overrightarrow{H}}^{T(A)}(B,C) = \min_{\tau \in A} \max_{b\in B} \min_{c\in C} \|b-(c+\tau)\|_{\infty} \leq \gamma.\]


Clearly, $\|b-(c+\tau)\|_{\infty} \leq \gamma$ if and only if for all dimensions $i \in \{1,\dots d\}$, we have $b[i] -(c[i]+\tau[i]) \leq \gamma$ and $(c[i]+\tau[i])-b[i]\leq \gamma. $
Thus, it remains to check 

\begin{align*}
\exists \tau \in A \forall b \in B \exists c \in C: \bigwedge_{i=1}^{d} b[i] -(c[i]+\tau[i]) \leq \gamma \land (c[i]+\tau[i])-b[i]\leq \gamma.
\end{align*}
\end{example}
\begin{example}[Triangle Detection]
\label{example:triangle}
Let $E$ be the set of edges in a directed graph. Each edge has an id and consider $\alpha,\omega$ to be functions that denote the start and endpoint of an edge respectively.
Thus $E'=\{(e_{id},\alpha(e),\omega(e)):e \in E\}$.
To detect a triangle we can simply ask 
\begin{align*}
\exists e_1 \in E \exists e_2 \in E \exists e_3 \in E:& e_1[0] \neq e_2[0] \land e_2[0] \neq e_3[0]\land e_1[0] \neq e_3[0] \land \\
&e_1[2]=e_2[1] \land e_2[2]=e_3[1] \land e_3[2]=e_1[1].
\end{align*}
Thus a $\Tilde{O}(n^{1+\epsilon})$ time algorithm for $3$-SUM implies a $\Tilde{O}(m^{1+\epsilon})$
time algorithm for triangle detection. 
\end{example}

Let us now take a look at the MaxConv lower bound problem (see Definition \ref{def:maxconvlb}).
\begin{lemma}
    The MaxConv lower bound problem is a member of the class $\mathsf{FOP}_{\mathbb{Z}}(\exists \forall \exists)$,
    and a member of the class $\mathsf{FOP}_{\mathbb{Z}}(\forall \exists \exists)$.
    \label{maxconvlb}
  \end{lemma}
  \begin{proof}
    \begin{enumerate}
  \item 
  Let 
  \begin{align*}
  &A'=\{ (A[i],i): i \in [n-1] \} \\
  &B'=\{(B[j],j): j\in [n-1] \} \cup \{(-M, -j): j \in \{1,\dots,n-1\} \}\\
  &C'=\{(C[k],k): k \in [n-1] \},
  \end{align*}
  where $M=3\cdot \max{(A\cup B \cup C)}.$
  We ask 
  $$\exists c' \in C' \forall a' \in A' \exists b' \in B': (i+j=k \land C'[k]>A'[i]+B'[j]).$$
  Thus, we can formulate MaxConv lower bound in $\mathsf{FOP}_{\mathbb{Z}}(\exists \forall \exists).$
  
  We give a short proof to this equivalence in the following. We have that $C[k]$ is a non witness to MaxConv lower bound if and only if  $\forall i \in [n-1]: C[k]>A[i]+B[k-i]$.
  Now, let us make a case distinction on $i$.
  Consider the case $i\leq k$, then only $j=k-i \in [n-1]$ fulfills $i+j=k$, and due to the fact 
  that $c[k]$ is a non witness $C[k]>A[i]+B[j]$.
  For the case $i>k$,  we have $j$ negative, which trivially fulfills $C[k]>A[i]+B[j]$.
  
  For the other direction notice that there exists a $k \in [n-1]$ which fulfills for all indices $i+j=k$ that $C[k]>A[i]+B[j]$.
  
  \item For the following constructed sets:
  \begin{align*}
  &A'=\{ (A[i],i): i \in [n-1] \}\\
  &B'=\{(B[j],j): j\in [n-1] \}\\
  &C'=\{(C[k],k): k \in [n-1] \} \cup \{(-M, k): k \in \{n,...,2n\} \},
  \end{align*}
  where $M=3\cdot \max A\cup B \cup C .$
  It can be easily seen that the following formula in $\mathsf{FOP}_{\mathbb{Z}}(\forall \exists \exists)$ models the MaxConv lower bound problem, 
  $$
  \forall c' \in C' \exists a \in A' \exists b' \in B': i+j=k \land C[k]\leq A[i]+B[j].
  $$
  \end{enumerate}
  \end{proof}
  The above Lemma presents a witness to the hardness of the classes $\mathsf{FOP}_{\mathbb{Z}}(\forall \exists \exists)$ and 
  $\mathsf{FOP}_{\mathbb{Z}}(\exists \forall \exists)$.
  


==> preliminaries.tex <==
\section{Preliminaries}\label{sec:prelim}
Let us first state problems and hypotheses we work with, starting with the $k$-SUM problem. 
\begin{definition}[The $k$-SUM problem]
Given $k$ finite sets of at most $n$ integers $A_1, A_2, \dots, A_k\subseteq \{-n^{k},\dots,0, \dots ,n^{k} \},$ and an integer $t$, determine if 
$\exists a_1 \in A_1 \exists a_2 \in A_2 \dots \exists a_k \in A_k: \sum_{i=1}^{k}a_i=t.$
\end{definition}

There is a simple meet-in-the-middle approach to solve the above problem in time $O(n^{\lceil k/2 \rceil+o(1)})$. It is widely
believed that this is optimal, as stated in the following hypothesis.
\begin{hypothesis}[The $k$-SUM Hypothesis]
Let $k\geq3$. There is no algorithm solving the $k$-SUM problem in time $O(n^{\lceil \frac{k}{2} \rceil -\epsilon})$ for any $\epsilon>0$.
\end{hypothesis}
For discussion of its plausibility, we refer to the survey \cite{williams2018some}.
We work in the standard word RAM model with words of $O(\log(n))$ bits. As we aim to relate runtime between quadratic time problems, we need 
a different notion of reduction than those used to prove NP completeness.

Fine-grained reductions were first introduced for subcubic runtimes in
\cite{DBLP:conf/focs/WilliamsW10}. A general definition can be found in \cite{williams2018some}.
In this paper, the following definition of fine-grained reduction, also used in \cite{DBLP:conf/approx/BringmannCFK21} suffices. A more detailed description on fine-grained reductions
can be found in \cite{DBLP:conf/innovations/CarmosinoGIMPS16}.

\begin{definition}[Fine-grained reductions]
Consider problems $P_1, P_2$ with presumed time complexities $T_1,T_2,$ respectively.
A fine-grained reduction from $P_1$ to $P_2$ is an algorithm $\mathcal{A}$ with oracle access to $P_2$. Whenever $\mathcal{A}$
uses an $O(T_2(n)^{1-\epsilon})$ algorithm for oracle calls to $P_2$ (for an $\epsilon>0$), there exists an $\epsilon'>0$,
such that $\mathcal{A}$ runs in time $O(T_1(n)^{1-\epsilon'})$. We write this as $(P_1,T_1) \leq (P_2,T_2).$
\end{definition}
We introduce for problems $P,Q$ the notation $P \leq_{c}Q$ if and only if $(P,n^c) \leq (Q,n^c)$ holds. Furthermore, $P$ and $Q$ are fine-grained equivalent, denoted by
$P \equiv_{c}Q$, if and only if $(P,n^c) \leq (Q,n^c)$ and $(Q,n^c) \leq (P,n^c) $ holds. We call $P_1,P_2$ subquadratic equivalent if $P_1 \equiv_2 P_2$.


A convolution of two vectors $x:=(x_0, \dots,x_{n-1})$ $y:=(y_0, \dots, y_{n-1})$
is defined as $z=(z_0, \dots,z_{2n-2})$, where $$z[k]:= \sum_{i,j \in [n-1], i+j=k} x_i \cdot y_j.$$ It is a well known fact that one can compute 
the sumset $A+B$ by computing the convolution of the characteristic vectors of $A$ and $B$.
In particular, we also make use of the theorem from Bringmann et al. \cite{DBLP:journals/corr/abs-2107-07625} on sparse convolutions.
\begin{theorem}
There is a deterministic algorithm to compute the convolution of two nonnegative vectors $A,B \in \mathbb{N}^n$ in time $O(t \text{polylog}(n \Delta)),$ where 
$t$ denotes the number of non-zero entries in the output convolution vector and $\Delta$ denotes the maximum entry size of the vectors $A,B$.
\label{sprase_conv}
\end{theorem}

The convolutional $3-$SUM problem asks for three sequences $A,B,C$ of size $n$, whether $\exists 0\leq i, j, k \leq n-1: a[i]+b[j]=c[k]$.
It is well known by a reduction from Pătrașcu \cite{DBLP:conf/stoc/Patrascu10} that there is no $O(n^{2-\epsilon})$ for an $\epsilon>0$ algorithm  for the Convolutional 3-SUM problem if and only if the 3-SUM hypothesis holds. 
The strong convolutional $3$-SUM hypothesis asks this question over a linearly sized universe \cite{DBLP:conf/icalp/AmirCLL14}, that is $A,B,C \subseteq \{-n,\dots,n\}.$ 


Let us fix the notation throughout the paper. We denote the sumset $U+V:= \{u+v: u \in U,v  \in V\}$. The $i$-th entry
of a vector $v$ is denoted by $v[i]$. For natural numbers $n$, we denote by $n[i]$ the $i$-th bit of $n$, where $n[0]$ is the least significant bit. Furthermore, we say the $i$-th bit of a natural number is set iff $n[i]=1.$
For vectors $u,v$ we write $u \leq v$ if and only if for all dimensions $i$ it holds that $u[i] \leq v[i]$. If $u \leq v$, we say $u$ is dominated by $v$.

For a unary function $f: U \to M$ and a set $A \subseteq U$ denote $f(A):= \{f(a): a\in A\}$. We abbreviate by $[t]:= \{0,\dots,t\}$. 
The notation $\Tilde{O}(T):=T \log^{O(1)}T$ is used
to hide poly-logarithmic factors. We denote the cardinality of a set $A$ by $\# A$ or $|A|$. Linear Integer arithmetic refers to the first order logic over the domain $\mathbb{Z}$ with
vocabulary: equality $(=)$,  inequality $(<,>,\geq,\leq)$,  and addition $(+)$. We use $\binom{V}{k}$ to denote all $k$-element subsets of $V$.

The $(M,d)$-vector $k$-SUM problem is defined as follows \cite{DBLP:journals/corr/AbboudLW13}.
For given $k$ sets $A_1 ,\dots ,A_k$ of size at most $n$ where each $A_i \subseteq \{-M,\dots, M\}^d$ and a target $t \in \{-M,\dots, M\}^d,$
do there exist $a_1 \in A_1, \dots, a_k \in A_k: a_1+\dots+ a_k=t$ 
Through the standard technique of interpreting vectors as integers we get:
\begin{lemma}
  The $(M,d)$-vector $k$-SUM problem can be reduced to the $k$-SUM problem with universe size $\{0,\dots, (kM+1)^d\}$ in time $O(n \log M).$
\label{trans_vec_to_k}
\end{lemma}
For a proof of the above see the proof of Abboud et al. \cite{DBLP:journals/corr/AbboudLW13} or our multiset adaptation of the proof in Lemma \ref{vector_to_one_red}.
A functional version of the $3$-SUM we will require is the following
\begin{definition}[All-ints $3$-SUM]
Given sets $A,B,C$ of at most $n$ integers $A,B,C \subseteq \{-n^k, \dots, n^k\}$ for each $a \in A$ determine,
whether there exist $b \in B$ and $c \in C$ such that $a+b+c=t$.
\end{definition}
\begin{lemma}[All-ints $3$-SUM $\equiv_2$ $3$-SUM \cite{DBLP:conf/focs/WilliamsW10}]
There exists a $O(n^{2-\epsilon})$ time algorithm for the All-ints $3$-SUM problem for an $\epsilon>0$
if and only if there exists a $O(n^{2-\epsilon'})$ time algorithm for $3$-SUM for an $\epsilon'>0$.
\label{allintsequiv}
\end{lemma}
For a proof see results from Williams et al. \cite{DBLP:conf/focs/WilliamsW10}.
It is known that the reduction can be made deterministic for instance using the $3$-SUM self reduction from Lincoln et al. \cite{DBLP:conf/icalp/LincolnWWW16} combined with the technique
introduced by Williams et al.\cite{DBLP:conf/focs/WilliamsW10}.
We continue with a $3$-SUM version, which aims to count witnesses.

  \begin{definition}[$\#3$-SUM]
    Given sets $A,B,C$ of at most $n$ integers $A,B,C \subseteq \{-n^k, \dots, n^k\}$.  The $\#3$-SUM problem asks for the number of triplets $(a,b,c) \in A \times B \times C$ such that $a+b+c=0$. \footnote{This version of $3$-SUM is equivalent to the version where $a+b+c=t$  for an integer $t$ is asked. In particular by setting $C':=C-\{t\}$, we get a reduction that preserves all solutions.}
    \end{definition}
  
  \begin{definition}[All-ints \#$3$-SUM]
    Given sets $A,B,C$ of at most $n$ integers $A,B,C \subseteq \{-n^k, \dots, n^k\}$. The All-ints $\#3$-SUM problem, asks to determine for each $a \in A$ the number of $(b,c) \in B \times C$ such that $a+b+c=0$.
  \end{definition}
    In our paper, we make use of the following recent powerful result from Chan et al. \cite{DBLP:journals/corr/abs-2303-14572}
    \begin{theorem}[\cite{DBLP:journals/corr/abs-2303-14572}]
    The following problems are all subquadratic equivalent
    \begin{itemize}
      \item $\#$All-ints $3$-SUM,
      \item $3$-SUM,
      \item $\#3$-SUM.
    \end{itemize}
    \label{Count3}
    \end{theorem}
As a remark, the non-trivial reductions rely on randomization techniques and to date it is not known whether it can be made deterministic.



    \begin{definition}[3-Uniform $k$-hyperclique problem]
      Given a $k$-partite 3-uniform hypergraph $G=(V,E)$, that is the vertices are a disjoint union of sets $V_1, V_2, \dots, V_k$ of size $n$ each, and $E$ is a set of edges
      of the form ${v_a,v_b,v_c}$ where $a,b,c$ are distinct and $v_a \in V_a, v_b \in V_b , v_c \in V_c$. The problem asks if there exists a $k-$Clique in $G$, that is vertices $v_1 \in V_1, \dots, v_k \in V_k$,
      such that for all $$a,b,c \in \binom{\{1,\dots,k\}}{3}$$ there exists an edge $\{v_a, v_b,v_c \}.$
      \end{definition}
      There is a naive algorithm deciding the above problem in $O(n^k)$. It is strongly believed
      that this runtime is optimal. One reason is that matrix multiplication techniques that speed up clique detections in graphs (rather than hypergraphs) 
      seem to fail, see for instance \cite{DBLP:conf/soda/LincolnWW18}. Furthermore, a faster algorithm would lead to an exponential improvement 
      over current $2^{n-o(n)}$ algorithms for MAX 3-SAT, see \cite{DBLP:conf/sat/ChenS15,DBLP:conf/focs/AlmanCW16}.
      Thus, we work with the following hypothesis.
      \begin{hypothesis}[3-Uniform Hyperclique Hypothesis]
      There is no $O(n^{k-\epsilon})$ algorithm solving the 3-Uniform $k$-hyperclique problem for $k\geq 4$ and an $\epsilon >0$. 
      \label{hyperclique_conj}
      \end{hypothesis}
    

      In \cite {DBLP:journals/talg/CyganMWW19}, Cygan et al. studied the MaxConv lower bound problem, but were unable to give a nontrivial upperbound.
      They managed to only show a reduction from this problem to the $L_p$ necklace alignment problem.
      The problem is defined as follows:
      \begin{definition}[MaxConv lower bound]
      \label{def:maxconvlb}
      Given integer arrays $A,B,C$ of length $n$. Determine whether 
      $C[k] \leq \max_{i+j=k} (A[i]+B[j])$ holds.
      \end{definition}


A key in our proofs will be a slightly generalized version of a lemma, whose aim it is to reduce inequality checking to a logarithmic amount of equality checks \cite{DBLP:journals/siamcomp/WilliamsW13}. 
\begin{lemma}[Bit-trick]
  For any non-negative integers $x_1,x_2, \dots, x_k, z \in \{0,\dots,U\},$ we have the following equivalence:
  \begin{align*}
      x_1+ \dots +x_k >z \iff & \text{There are } \ell \in \{1,\dots, [\lceil \log_2(U) \rceil] \}, b\in \{1,2, \dots, k\}:\\
      & pre_\ell(x_1)+\dots +pre_\ell(x_k)=pre_\ell(z)+b,
  \end{align*}
  where $pre_\ell(x)$ denotes the number remaining when taking the first $l$ bits of $x$, where the most significant bit is considered the first bit. Formally, for $z \in \{0,\dots,U\}$ and $\ell \in \{0,\dots, \lceil \log_2(U) \rceil\}$ $pre_\ell(z):=\lfloor \frac{z}{2^{B-\ell}} \rfloor,$ where $B$ denotes the number of bits in $z$.
  \label{bit_trick}
  \end{lemma}
  \begin{proof}
    If  $pre_\ell(x_1)+pre_\ell(x_2)+ \dots +pre_\ell(x_k)=pre_\ell(z)+b$, for $B$-bit integers holds, we have
    \begin{align*}
       & \sum_{i=B-\ell}^{B-1}2^{i}x_{1}[i] + \dots +\sum_{i=B-l}^{B-1}2^{i}x_{k}[i]  = \sum_{i=B-\ell}^{B-1}2^{i}z[i]+2^{B-l}b \\
        \implies &\sum_{i=B-\ell}^{B-1}2^{i}(x_1[i]+x_2[i] +\dots + x_k[i]) =\sum_{i=B-\ell}^{B-1}2^{i}z[i]+2^{B-l}b\\
        \implies & \sum _{i=1}^k x_i=z+ \sum_{i=0}^{B-\ell-1}(x_1[i]+x_2[i] +\dots + x_k[i]-z[i])+2^{B-\ell}b\\
        \implies &\sum _{i=1}^k x_i >z.
    \end{align*}
    Assume now that $x_1+x_2 + \dots + x_k >z$ holds, let $$ \hat{\ell} :=\min\{i:1\leq i\leq B \land  pre_i(x_1)+pre_i(x_2)+\dots +pre_i(x_k)>pre_i(z)\}. $$ If $b \leq k$, the statement holds, for the sake of a contradiction assume $$pre_{\hat{\ell}}(x_1)+ pre_{\hat{\ell} }(x_2)+ \dots + pre_{\hat{\ell} }(x_k) \geq pre_{\hat{\ell} }(z)+k+1. $$
    We know that the following holds for any $B$-bit integer $x$ and any $1 \leq l\leq B$
    $$2pre_{\ell-1}(x) \leq pre_\ell(x) \leq 2pre_{\ell-1}(x)+1. $$
    Thus, we have
    \begin{align*}
        2\left(pre_{\hat{\ell} -1}(x_1)+ \dots + pre_{\hat{\ell} -1}(x_k)   \right) +k & \geq  pre_{\hat{\ell} }(x_1)+ \dots + pre_{\hat{\ell}}(x_k) \\
        & \geq pre_{\hat{\ell} } (z) +k +1\\
        & \geq 2pre_{\hat{\ell} -1}(z)+k+1 .
        \end{align*}
    Concluding $$ pre_{\hat{\ell} -1}(x_1)+ pre_{\hat{\ell} -1}(x_2)+ \dots + pre_{\hat{\ell} -1}(x_k)  \geq pre_{\hat{\ell} -1}(z) +1/2,$$ and thereby also
    $$ pre_{\hat{\ell} -1}(x_1)+ pre_{\hat{\ell} -1}(x_2)+ \dots + pre_{\hat{\ell} -1}(x_k)   > pre_{\hat{\ell} -1}(z), $$ contradicting the minimality of $\hat{\ell} $.
    \end{proof}
We conclude this section with an observation.
\begin{observation}
 The choices of $\ell$ and $b$ in Lemma \ref{bit_trick} are not unique, but there is a unique $\ell \in \{1,\dots, \lceil \log_2(U) \rceil \}$ and $b \in \{1,\dots,k\}$ such that the following holds
 \begin{align*}
  \sum_{i=1}^{k}x_i >z \iff \sum_{i=1}^{k}pre_\ell(x_i)=pre_l(z)+b \land \sum_{i=1}^{k}pre_{\ell-1}(x_i)=pre_{\ell-1}(z).
 \end{align*}
 \label{uniqueness_bit}
\end{observation}

